Nearly Consistent Finite Particle Estimates in Streaming Importance Sampling

In Bayesian inference, we seek to compute information about random variables such as moments or quantiles on the basis of {available data} and prior information. When the distribution of random variables is {intractable}, Monte Carlo (MC) sampling is usually required. {Importance sampling is a standard MC tool that approximates this unavailable distribution with a set of weighted samples.} This procedure is asymptotically consistent as the number of MC samples (particles) go to infinity. However, retaining infinitely many particles is intractable. Thus, we propose a way to only keep a \emph{finite representative subset} of particles and their augmented importance weights that is \emph{nearly consistent}. To do so in {an online manner}, we (1) embed the posterior density estimate in a reproducing kernel Hilbert space (RKHS) through its kernel mean embedding; and (2) sequentially project this RKHS element onto a lower-dimensional subspace in RKHS using the maximum mean discrepancy, an integral probability metric. Theoretically, we establish that this scheme results in a bias determined by a compression parameter, which yields a tunable tradeoff between consistency and memory. In experiments, we observe the compressed estimates achieve comparable performance to the dense ones with substantial reductions in representational complexity.

==> Applications.tex <==
%\vspace{-3mm}
\section{Application and Numerical tests}\label{sec:fields}
\subsection{Classification with Fairness Constraints}



With the increase in the process of automated decision making and the size of analyzed data becomes large there are growing concerns from government, civil organization and researchers \cite{sweeney2013discrimination} that automated decision can lead to loss of fairness, transparency and accountability. As algorithmic decision making process replaces human supervision and are becoming data driven, even in
the absence of intent, they can be unfair. To evaluate the fairness of a decision making process authors in \cite{zafar2015fairness} introduced the notion of disparate impact. A decision making process has disparate impact if it outcomes unfairly benefit (or hurt) particular groups of people with similar sensitive attributes such as race and sex. We will use $p$\% rule to quantify disparate impact as mentioned in \cite{zafar2015fairness}. Basically the $p$\%-rule states that the ratio
between the percentage of examples with a certain
sensitive attribute value classified as positive  in decision
outcome and the percentage of examples without 
that value also classified as positive must not 
be less than $p:100$. 

In binary classification, the primary task is to learn a mapping function $f(\bbx)$ between feature vectors $\bbx \in \mathcal{R}^d$ and class labels $y \in \{-1,1\}$, using available training data set $[\bbx_i,y_i]^N_{i=1}$.  Typically the target is to obtain a decision boundary, characterized by a set of parameters $\bbtheta^*$, which gives the highest classification accuracy for the test data set, by minimizing a loss function $L(\bbtheta)$ over the training set. Let $r_{\bbtheta^*}(\bbx)$ be the distance between decision boundary and feature vector $\bbx$. For any new example $\bbx_i$ from test set, the classifier will predict $f_{\bbtheta}(\bbx_i)=1$ if  $r_{\bbtheta^*}(\bbx_i)\geq 0$ and $f_{\bbtheta}(\bbx_i)=-1$ for $r_{\bbtheta^*}(\bbx_i)< 0$. However, if class labels of training examples are correlated with sensitive attribute $\{\bbs_i\}_{i=1}^N$, then the classifier may suffer from disparate impact. That is the percentage of examples having a certain sensitive
attribute  with $r_{\bbtheta^*}(\bbx)\geq 0$ may differ dramatically
from the percentage of examples without this sensitive attribute having $r_{\bbtheta^*}(\bbx)\geq 0$\cite{zafar2015fairness}. 
%It must be noted that even if the decision boundary is determined without %using sensitive attributes, this may
%happen  if  it is correlated with
%one or more features, through indirect discrimination [].



 We intend to design a classifier which
maximizes accuracy under the fairness constraints. In order to measure  the fairness/unfairness of decision boundary we define the covariance between the sensitive
attributes $\{\bbs_i\}_{i=1}^N$, and  the distance $\{r_{\bbtheta}(\bbx)\}_{i=1}^{N}$ between decision boundary and feature vector as:
\begin{align}
Cov(\bbs,r_{\bbtheta}(\bbx))&= \mbE[(\bbs-\bar{\bbs})r_{\bbtheta}(\bbx)]-\mbE[(\bbs-\bar{\bbs})]\bar{r}_{\bbtheta}(\bbx)\nonumber\\
&\approx \frac{1}{N} \sum_{i=1}^{N} (\bbs_i-\bar{\bbs})r_{\bbtheta}(\bbx_i).
\label{Cov_intro}
\end{align} 

Now to incorporate the fairness constraint we can formulate the problem as follow:
 
 \begin{align}
&\bbtheta^*:=\argmin_{\bbtheta} L(\bbtheta)\nonumber\\
&\text{s.t.}\;\;\; \frac{1}{N}\sum_{i=1}^{N}(\bbs_i-\bar{\bbs})r_{\bbtheta}(\bbx_i)\leq \bbc\nonumber\\&\;\;\;\;\;\
\frac{1}{N}\sum_{i=1}^{N}(\bbs_i-\bar{\bbs})r_{\bbtheta}(\bbx_i)\geq -\bbc,
\label{app_prob_intro}
\end{align}
here $\bbc$ is the covariance threshold. Basically, $\bbc$ presents a 
trade off between fairness and accuracy, such that decreasing $\bbc$  towards zero, results in classifier with a larger p\%-rule but with a larger loss in accuracy. In this work we will use logistic regression
classifier, whose mapping function is given by the following probability distribution:
\begin{align}
\label{logistic_distribution}
p(y_i=1|\bbx_i,\bbtheta)=\frac{1}{1+e^{-\theta^T\bbx_i}},
\end{align}
here, we obtain $\bbtheta$ by solving $\argmin_{\theta}-\sum_{i=1}^{N} \log(p_i|\bbx_i,\bbtheta)$ over the training set. Thus problem \eqref{app_prob_intro} becomes:

\begin{align}
&\min_{\bbtheta} \;\;\;\frac{-1}{N}\sum_{i=1}^{N}\log{p(y_i|\bbx_i,\bbtheta)}\nonumber\\
&\text{s.t.}\;\;\; \frac{1}{N}\sum_{i=1}^{N}(\bbs_i-\bar{\bbs})\bbtheta^T\bbx_i\leq \bbc\nonumber\\&\;\;\;\;\;\
\frac{1}{N}\sum_{i=1}^{N}(\bbs_i-\bar{\bbs})\bbtheta^T\bbx_i\geq -\bbc.
\label{app_prob_main}
\end{align}

Here, we have chosen the decision boundary simply the hyperplane defined by $\bbtheta^T\bbx+b=0$. Further, we appended 1 to all feature vectors reducing the decision boundary from $\bbtheta^T\bbx+b=0$ to $\bbtheta^T\bbx=0$. From \eqref{stochastic_lagrangian} and \eqref{app_prob_main} we can  
define Lagrangian for $k^{th}$ realization of $y$ and $\bbx$ as:

\begin{align}
\hat{\mathcal{L}}_k(\bbtheta,\bblam)=&-\log p(y_k|\bbx_k,\bbtheta)+\lam_1\big((\bbs_k-\bar{\bbs})\bbtheta^T\bbx_k-\bbc\big)\nonumber\\&-\lam_2\big((\bbs_k-\bar{\bbs})\bbtheta^T\bbx_k+\bbc\big)-\frac{\delta}{2}\eps_k(\lam_1^2+\lam_2^2).
\label{app:lagrangian}
\end{align}


\begin{figure}[!tbp]
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{Obj_syn}
    \caption{Objective}
    \label{obj_syn}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{CV_syn}
    \caption{Constraint violation}
    \label{vio_syn}
  \end{subfigure}
  \caption{Convergence results on Synthetic Data set}
\end{figure}

\begin{figure}
	\centering
	\setcounter{subfigure}{0}
	\begin{subfigure}{0.7\columnwidth}		\includegraphics[width=\linewidth, height = 0.6\linewidth]{scatter_pi4}
		\caption{$\phi/4$}
		\label{scatter_pi4}
	\end{subfigure}\hspace{2.8cm}
	\begin{subfigure}{0.7\columnwidth}
		\includegraphics[width=\linewidth, height = 0.6\linewidth]{scatter_pi8}
		\caption{$\phi/8$}
		\label{scatter_pi8}
	\end{subfigure}
	\caption{Plots for synthetic data: For the scatter plot shown in (a) and (b), the solid light blue lines show the decision boundaries for unconstrained case. The dashed lines show the decision boundaries trained to maximize accuracy under fairness constraints.}
	\label{results_syn}
	\vspace{-0mm}
\end{figure}

\begin{figure*}
	\centering
	\setcounter{subfigure}{0}
	\begin{subfigure}{0.6\columnwidth}		\includegraphics[width=\linewidth, height = 0.6\linewidth]{p_vs_c_syn}
		\caption{p\%-rule vs. Cov.}
		\label{P_C_SYN}
	\end{subfigure}\hfill
	\begin{subfigure}{0.6\columnwidth}
		\includegraphics[width=\linewidth, height = 0.6\linewidth]{acc_vs_p_syn}
		\caption{Accuracy vs. p\%-rule}
		\label{A_P_SYN}
	\end{subfigure}\hfill
	\begin{subfigure}{0.6\columnwidth}
		\includegraphics[width=\linewidth, height = 0.6\linewidth]{z_vs_c_syn}
		\caption{\% in Positive class vs. Cov.}
		\label{Z_C_SYN}
	\end{subfigure}
	\caption{Panel (a) shows the correspondence between the
covariance and the p\%-rule for classifiers trained under fairness constraints. Panel (b) shows the accuracy
against p\%-rule value. Panel (c) shows the percentage of protected and non-protected examples in the
positive class against the covariance }
\label{SYN}
	\vspace{-0mm}
\end{figure*}

%From \eqref{iterate_primal} and \eqref{iterate_dual} primal and dual updates are:
%
%\begin{align} \label{app_iterate_primal}
%\bbtheta_{k+1}   &=\ccalP_{\ccalX}\Big[ \bbtheta_k - \eps_k \nabla_{\bbtheta} \hat{\ccalL}_k (\bbtheta_k, \bblam_k)\Big] \;,  \\
%\bblam_{k+1} &= \Big[\bblam_k + \eps_k \nabla_{\bblam} \hat{\ccalL}_k (\bbx_{k}, \bblam_k)  \Big]_+\;
%\label{app_iterate_dual}
%\end{align}
%
%Computing gradients:
%
%\begin{align}
%\nabla_{\bbtheta}& \hat{\ccalL}_k (\bbtheta_k, \bblam_k)=\nonumber\\&-\nabla_{\bbtheta} \big(\log p(y_k|\bbx_k,\bbtheta)\big)+(\lam_{k,1}-\lam_{k,2})(\bbz_k-\bar{\bbz})\bbx_k
%\label{app:grad_theta}
%\end{align}
%For $p(y_i=1|\bbx_i,\bbtheta)=1/(1+e^{-\bbtheta^T\bbx_i})$
%\begin{align}
%\nabla_{\bbtheta_j} \big(\log p(y_k|\bbx_k,\bbtheta_j)\big)=\frac{\bbx_{k,j}}{1+e^{\bbtheta_j \bbx_{k,j}}}; \;\;\;j=1,2
%\end{align}
%
%For $p(y_i=-1|\bbx_i,\bbtheta)=1-\big(1/(1+e^{-\bbtheta^T\bbx_i})\big)$
%\begin{align}
%\nabla_{\bbtheta_j} \big(\log p(y_k|\bbx_k,\bbtheta_j)\big)=\frac{-\bbx_{k,j}e^{\bbtheta_j \bbx_{k,j}}}{1+e^{\bbtheta_j \bbx_{k,j}}}; \;\;\;j=1,2
%\end{align}
%
%Similarly
%\begin{align}
%\nabla_{\bblam_{1}}& \hat{\ccalL}_k (\bbtheta_k, \bblam_k)=(\bbz_k-\bar{\bbz})\bbtheta^T\bbx_k-\bbc-\delta \eps_k \lam_1
%\end{align}
%
%and 
%\begin{align}
%\nabla_{\bblam_{2}}& \hat{\ccalL}_k (\bbtheta_k, \bblam_k)=-(\bbz_k-\bar{\bbz})\bbtheta^T\bbx_k-\bbc-\delta \eps_k \lam_2
%\end{align}




\begin{figure*}
	\centering
	\setcounter{subfigure}{0}
	\begin{subfigure}{0.6\columnwidth}		\includegraphics[width=\linewidth, height = 0.6\linewidth]{p_vs_c_adult_compare}
		\caption{p\%-rule vs. Cov.}
		\label{P_adult}
	\end{subfigure}\hfill
	\begin{subfigure}{0.6\columnwidth}
		\includegraphics[width=\linewidth, height = 0.6\linewidth]{acc_adult_compare}
		\caption{Accuracy vs. p\%rule}
		\label{acc_adult}
	\end{subfigure}\hfill
	\begin{subfigure}{0.6\columnwidth}
		\includegraphics[width=\linewidth, height = 0.6\linewidth]{time_compare_adult}
		\caption{Time variation with Sample size}
		\label{time}
	\end{subfigure}
	\caption{Results on Adult Dataset[]: Panel (a) shows variation of P\% with Covariance, (b) shows the accuracy
against p\%-rule, (c) shows the variation of time required by algorithm with increase in sample size of synthetic data.}
\label{compare}
	\vspace{-0mm}
\end{figure*}


For the simulation purposes we will use both the synthetic and real world data. We will show that the formulation in \eqref{app_prob_main} allows us to finely control the fairness, at a small loss in accuracy of the classifier.
\subsubsection{Synthetic data} We generate synthetic data the same way as mentioned in \cite{zafar2015fairness}. Total 4000 binary labels are generated uniformly at random. Two different Gaussian distributions are generated as: $p(x|y=1)=N([2;2],[5, 1;1, 5])$ and $p(x|y=-1)=N([-2;-2],[10, 1;1, 3])$. The feature vectors are assigned to labels by drawing samples from above two distributions.  For sensitive attribute $s$ we have used Bernoulli distribution: $p(s=1)=p(\hat{\bbx}|y=1)/p(\hat{\bbx}|y=1)+p(\hat{\bbx}|y=-1)$, here $\hat{\bbx}=[\cos(\phi), -\sin(\phi);\sin(\phi), \cos(\phi)]$. The correlation between sensitive attribute and class labels (i.e. disparate impact) depends on the parameter $\phi$. The smaller the $\phi$, the higher the correlation. In Fig. \ref{results_syn}- Fig. \ref{SYN}, we plot the results of this numerical experiment. 

%\begin{figure}
%	\centering
%	\setcounter{subfigure}{0}
%	\begin{subfigure}{0.8\columnwidth}		\includegraphics[width=\linewidth, height = 0.6\linewidth]{Obj_adult}
%		\caption{Objective vs. iteration $k$}
%		\label{obj_adult}
%	\end{subfigure}\hspace{2.8cm}
%	\begin{subfigure}{0.8\columnwidth}
%		\includegraphics[width=\linewidth, height = 0.6\linewidth]{CV_adult}
%		\caption{Constraint violation vs. iteration $k$ }
%		\label{vio_adult}
%	\end{subfigure}
%	\caption{For Adult dataset}
%	\vspace{-0mm}
%\end{figure}



\begin{figure}[!tbp]
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{Obj_adult}
    \caption{Objective }
    \label{obj_adult}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.24\textwidth}
    \includegraphics[width=\textwidth]{CV_adult}
    \caption{Constraint violation }
    \label{vio_adult}
  \end{subfigure}
  \caption{Convergence results on Adult Data set}
\end{figure}



Fig. \ref{obj_syn} shows the objective $(1/N)\sum_{i}\mbE_{\bbtheta_i}f(\bbx,\bbtheta_i) $
versus iteration k. In Fig. \ref{vio_syn}, we plot the constraint violation graph. The decision boundaries generated by the
classifiers for maximizing accuracy with fairness constraints is shown in Fig.\ref{scatter_pi4}-\ref{scatter_pi8}. The unconstrained
decision boundary is represented by a solid line while boundaries for different covariance thresholds, c is shown in dotted line. It can be observed that incorporating fairness constraint in data generation process, results into the rotation of the decision boundary (compared to unconstrained boundary). The rotation is more as the threshold value c is decreased. Fig.\ref{scatter_pi4} and Fig.\ref{scatter_pi8} also shows that increase in the correlation in the data i.e. chaining $\phi$ from $\pi/4$ to $\pi/8$ causes more rotation. Additionally, in Fig.\ref{SYN} we investigates the relation between p\% rule, accuracy and covariance. Fig.\ref{P_C_SYN} shows that higher the covariance, the lower the p\%-
rule the classifier satisfies. Moreover, Fig.\ref{A_P_SYN} shows the trade-off between p\% rule and accuracy: more p\% (i.e. smaller covariance or a larger rotation) leads to a more fair solution, but at the cost of reduced accuracy. In Fig.\ref{Z_C_SYN} we plotted  the percentage of protected and non-protected examples in the positive class against the covariance. It shows that to achieve more fairness (i.e. reduced cov or increased p\% rule) classifier moves more non-protected examples to negative class and protected examples to positive class. These results shows that the problem formulation of \eqref{app_prob_main} successfully incorporates fairness constraint by exploiting the covariance defined in \eqref{Cov_intro} and allows to control fairness constraint with small loss in accuracy.

\subsubsection{Real data}
We experiment with the Adult income dataset []. It has a total of
45222 examples, each with 14 features like education level, age, marriage status. The label (binary), denotes which subject has income  (positive class) or less (negative class) than 50K \$ . We have considered sex as a binary sensitive attribute. We refer females as protected group while
males as non-protected groups. In our experiments, we use 70\% of data for training while rest (30\%) are used for testing. We repeat our experiment 5 times and all the reported results are average of this.

The plot of objective and constraint violation versus iteration is shown in Fig.\ref{obj_adult} and Fig.\ref{vio_adult} respectively. We compare our approach to method presented in \cite{zafar2015fairness}. Fig.\ref{P_adult} shows variation of p\%-rule with covariance, as expected reducing covariance results in higher p\% value. Also it establishes that our proposed algorithm shows almost same p-\% value as that of \cite{zafar2015fairness} for different covariance values.  The accuracy (Fig.\ref{acc_adult}) of our algorithm although slighlty low, is comparable to  method presented in \cite{zafar2015fairness}. But the major advantage of proposed algorithm is in terms of time taken. As shown in Fig.\ref{time} our method clear has an advantage in terms of time as compared to method in \cite{zafar2015fairness}.






==> Convergence.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%S  E  C  T  I  O  N %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Balancing Consistency and Memory}\label{sec:convergence}
%
%\textcolor{blue}{In a lot of places we wrote $\bbx^n$ rather than $\bbx^{(n)}$. Please double check to make sure I corrected them all, especially in the proofs in appendices. \\  \\
%
%\textcolor{blue}{Also please check that I didn't screw up the difference between $\mu$, $\pi$, $q$, and $m$ and their respective tilde/hat versions.
%}

In this section, we characterize the convergence behavior of our posterior compression scheme. Specifically, we establish conditions under which the asymptotic bias is proportional to the kernel bandwidth and the compression parameter using posterior distributions given by Algorithm \ref{alg:compressed_online_kernel_importance_sampling}. To frame the discussion, we note that the pure SNIS estimator \eqref{eq:SNIS_estimator} $I_N(\phi)$, whose particle complexity goes to infinity, is asymptotically consistent \cite{mcbook}[Ch. 9, Theorem 9.2], %, i.e.,
%
%%
%\begin{align}\label{eq:consistent}
%%
% \mathbb{P}\left(\lim_{N\rightarrow \infty}I_N(\phi)= I(\phi) \right)=1 .%, \quad \Var(\hat{I})=\mathbb{E}\left[  \right]
%\end{align}
%%
and that the empirical posterior $I_N(\phi)$ contracts to its population analogue at a $\ccalO(1/N)$ rate where $N$ is the number of particles. To establish consistency, we first detail the technical conditions required. 
%detailed in Appendix \ref{apx_technicalities} are required.
\subsection{Assumptions and Technicalities}\label{apx_technicalities}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}\label{as:first}
%
Recall the definition of the target distribution $q$ from Sec. \ref{sec:prob} following \eqref{eq:posterior}. Denote the integral of test function $\phi:\ccalX \rightarrow \reals$ as $q(\phi)$. 
%
\begin{enumerate}[label=(\roman*)]
%
\item Assume that $\phi$  is absolutely integrable, i.e., $q(|\phi|)<\infty$, and has absolute value at most unit $|\phi|\leq 1$. \label{as:testfunction1}
%
\item The test function has absolutely continuous second derivative, and $\int_{\bbx\in\ccalX} \phi''(\bbx) d\bbx < \infty$. \label{as:testfunction2}
%
\end{enumerate}
%
\end{assumption}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assumption}\label{as:2}
The kernel function associated with RKHS is such that  $\int_{\bbx \in \ccalX} \kappa_{\bbx^{(n)}}(\bbx) = 1$,  $\int_{\bbx \in \ccalX} \bbx \kappa_{\bbx^{(n)}} (\bbx) = 0$, and $\sigma_{\kappa}^2 = \int_{\bbx \in \ccalX} \bbx^2 \kappa_{\bbx^{(n)}}(\bbx) >0$.
\end{assumption}

\blue{\begin{assumption}\label{as:approximation}
Let $I_{1}(\phi)$ and $I_{2}(\phi)$ be two integral estimators for test function $\phi$, the we define the approximation error for $\phi\notin\mathcal{F}$ where  $\mathcal{F}:=\{f\in\mathcal{H}~|~ \|f\|_{\mathcal{H}}\leq 1\}$, as 
%
 	 \begin{align}\label{approximation}
	I(\phi,f)= &\sup_{|\phi| \leq 1,f \in \mathcal{F}} \left(\mathbb{E}[I_1(\phi) \!-\! {I_2(\phi)}] \right)-\left(\mathbb{E}[ I_1(f) \!-\! {I_2(f)}] \right),
\end{align}
%
and we assume that $I(\phi,f)\leq \mathcal{Z}$, where $\mathcal{Z}$ is a finite constant.
\end{assumption}}
\red{skeptical about the above assumption}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{assumption}\label{as:last}
%\red{Denote as $\hat{m}$ and $\tilde{m}$ the mean embeddings (which belongs to $\ccalH$) of distributions $\hat{\rho},\tilde{\rho}$ \cite{sriperumbudur2010hilbert}} given by
%%
%\red{$$ \hat{m}=\mathbb{E}_{\hat{\rho}}[ \kappa_{\bbx}(\cdot) ] \; , \qquad \tilde{m} = \mathbb{E}_{\tilde{\rho}}[ \kappa_{\bby}(\cdot) ].$$}
%%
%%
%\red{The {'dist'} distance between the full distributions lower-bounds the distance between their mean embeddings: $dist(\hat{\rho},\tilde{\rho}) \leq  \| \hat{m} - \tilde m \|_{\ccalH}$, which are related by a multiplicative factor $dist(\hat{\rho},\tilde{\rho})  = K \| \hat{m} - \tilde m \|_{\ccalH}$.}
%%
%\end{assumption}
%
%
%\blue{need some comments about assumptions}
Assumption \ref{as:first}\ref{as:testfunction1} is a textbook condition in the analysis of Monte Carlo methods, and appears in \cite{mcbook}. Assumption \ref{as:first}\ref{as:testfunction2} and \ref{as:2} are required conditions for establishing consistency of kernel density estimates and are standard -- see \cite{wasserman2006all}[Theorem 6.28]. 
%Assumption \ref{as:last} is {reasonable} considering the fact that a distribution is completely characterized by its moments \cite{durrett2019probability}. Hence if the full distribution is close according to some metric, then the moments are close -- see \cite{scholkopf2015computing}[eqn. (14)]. This assumption formalizes this statement for  means and metrics in RKHSs \cite{sriperumbudur2010hilbert}.
%
 We begin by noting that under Assumption \ref{as:first}, we have classical statistical consistency of importance sampling as the number of particles becomes large as stated in Lemma \ref{first_theorem} in Appendix \ref{first_proof}.
%
%The proof is in Appendix \ref{first_proof}. 
%
This result permits characterizing the bias of Algorithm \ref{alg:compressed_online_kernel_importance_sampling} given next. \blue{The Assumption \ref{as:approximation} here non-standard which is used to bound the error due to operating in the RKHS. We note that if $\phi\in\mathcal{F}$ which is the case for most of the practical applications [\red{citations}], the value of $\mathcal{Z}$ would exactly be  $0$. }
%\blue{we need to state some assumptions here}
%
%

\blue{\begin{lemma}\label{intermidiate_lemma}
Define the second moment of the true unnormalized density $\rho$ as in Lemma \ref{first_theorem}. Then, under Assumptions \ref{as:first}-\ref{as:approximation}, the estimator of Alg. \ref{alg:compressed_online_kernel_importance_sampling} satisfy
%
\begin{align}\label{lemma}
	%
	\big|\sup_{|\phi| \leq 1}  \big(\mathbb{E}[\hat I_N(\phi)- I(\phi)] \big) \big| \leq  \sum_{n=1}^{N}\epsilon_n+\frac{24}{N} \rho +\mathcal{Z}.
	%
\end{align}
%
where $\epsilon_n$ is the compression budget for each $n$.
\end{lemma}}

\begin{myproof}
	\blue{Inspired by \cite{agapiou2017importance}, begin by denoting $\hat I_N(\phi)$ as the integral estimate given by Algorithm \ref{alg:compressed_online_kernel_importance_sampling}. Consider the bias of the integral estimate ${\hat I_N(\phi) - I(\phi)}$, and add and subtract $I_N(\phi)$, the uncompressed self-normalized importance estimator, the result of Algorithm \ref{alg:importance_sampling}, i..e., we get}
	%
	\begin{align}\label{new}
		\hat I_N(\phi) - I(\phi)=& \hat I_N(\phi) -I_N(\phi)+I_N(\phi) - I(\phi).
	\end{align}
	%
	%where $\tilde I_N(\phi)$ is the uncompressed integral estimation at $N$ (\red{We might need to define it properly because without intorducing the kernalized IS, we have directly introduced the compressed kernelized density in Algorithm \ref{alg:compressed_online_kernel_importance_sampling}.}) $I_N(\phi)$ is the integral estimation given by Algorithm \ref{alg:importance_sampling}.  
	%
	Take the expectation on both sides with respect to the population posterior \eqref{eq:posterior} to obtain
	%
	\blue{\begin{align}\label{new2}
			\mathbb{E}[\hat I_N(\phi) - I(\phi)]=& \mathbb{E}[\hat I_N(\phi) -  I_N(\phi)]+\mathbb{E}[I_N(\phi) - I(\phi)].
	\end{align}}
	%
	%where we add and subtract $\mathbb{E}[I(\phi)]$ inside the second-to-last term and group like terms.
	%
	Let's compute the $\sup$ of both sides of \eqref{new2} over range $|\phi | \leq 1$ followed by fact that a sup of a sum is upper-bounded by the sum of individual terms:
	%
	%Using the triangle inequality, we can write 
	%
	\begin{align}\label{new3}
		%
		\sup_{|\phi | \leq 1} \left(\mathbb{E}[\hat I_N(\phi) - I(\phi)] \right)&\leq  \sup_{|\phi | \leq 1} \left(\mathbb{E}[\hat I_N(\phi) -  I_N(\phi)] \right)\nonumber
		\\
		%& + \sup_{|\phi | \leq 1} \left(\mathbb{E}[\tilde I_N(\phi)-I(\phi)]\right) \nonumber \\
		&\quad+\! \sup_{|\phi| \leq 1}\!\!\left([\mathbb{E}[I_N(\phi) \!-\! I(\phi\!)] \right)\!.
		%
	\end{align}
	%
	Now, compute the absolute value of both sides of \eqref{new3}, and to the last two terms, pull the absolute value inside the supremum.
	%
	%$$|\sup \left(\mathbb{E}[\tilde I_N(\phi)-I_N(\phi)]\right)  | \leq  \sup \left|\mathbb{E}[\tilde I_N(\phi)-I_N(\phi)]\right|.$$
	Then, \eqref{eq:posterior_contraction} (Lemma \ref{first_theorem}) applied to the last term yields: 
	%
	\begin{align}\label{new4}
		%
		\big|\sup_{|\phi| \leq 1}  \big(\mathbb{E}[\hat I_N(\phi)- I(\phi)] \big) \big| \leq & \left|\!\sup_{|\phi| \leq 1} \left(\mathbb{E}[\hat I_N(\phi) \!-\!  {I_N(\phi)}]\! \right)\!\right|\nonumber
		\\
		&+\frac{24}{N} \rho.
		%
	\end{align}
	%
	Thus, it remains to characterize the first term on the right-hand side of \eqref{new4},
	%We first focus on the second term $|\mathbb{E}[\tilde I_N(\phi)-I(\phi)]|$, which is the bias due to kernel smoothing. \cite{wasserman2006all}[Theorem 6.28] establishes this bias as
	%%
	%\begin{align}\label{eq:kernel_smoothing_bias}
	%%
	%\mathbb{E}[(\tilde I_N(\phi)-I(\phi))^2]&=\frac{1}{4}\sigma_{\kappa}^4 h^4 \phi''(\bbx)  + \frac{1}{hN} \nonumber \\
	%&\qquad+ \ccalO\left(\frac{1}{N}\right) + \ccalO(h^6).
	%\end{align}
	%%
	% Apply Jensen's inequality to pull the square outside the expectation, and compute the square root of both sides to obtain an upper-estimate of the bias of  $|\mathbb{E}[\tilde I_N(\phi)-I(\phi)]|$:
	% %
	%\begin{equation}\label{eq:kernel_smoothing_bias}
	%%
	%|\mathbb{E}[(\tilde I_N(\phi)-I(\phi))]|\!\lesssim\! \ccalO\left(\!\!\sigma_{\kappa}^2 h^2\!+\!\frac{1}{\sqrt{N h}}\!+\! \ccalO\!\!\left(\!\frac{1}{\sqrt{N}}\!\right)\!+\!h^3\!\!\right).
	%\end{equation}
	%%
	which is the integral approximation error associated using the compressed integral estimation via kernel mean embedding. \blue{
		% 	Let us denote the compressed posterior distribution at $N$ as $\hat\mu_N$ which we obtain by solving the pre-image problem in \eqref{eq:proximal_hilbert_representer} using the corresponding compressed kernel mean embedding $\beta_{\mu_N}$.  The compressed integral estimation $\hat I_N(\phi)$ is calculated using the compressed posterior distribution $\hat\mu_N$ and the uncompressed integral estimation $I_N(\phi)$ is calculated using the uncompressed posterior distribution denoted by $\nu_N$.
		To proceed with the analysis, let us add subtract the supremum over the space $\mathcal{F}:=\{f\in\mathcal{H}~|~ \|f\|_{\mathcal{H}}\leq 1\}$ 
		to the first term on the right hand side of \eqref{new4}, we get 
		%
		\begin{align}\label{IPM0}
			\sup_{|\phi| \leq 1} \left(\mathbb{E}[\hat I_N(\phi) \!-\! {I_N(\phi)}] \right)
			=&\sup_{f \in \mathcal{F} }\left(\mathbb{E}[\hat I_N(f) \!-\! {I_N(f)}] \right)\nonumber
			\\
			&+I(\phi,f),
		\end{align}
		where $I(\phi,f)$ is defined in \eqref{approximation}. %  	%
		% 	 where we define $I(\phi,f)$ as approximation error due $\phi(\bbx)$ not being in $\mathcal{F}$ as
		% 	 %
		% 	 \begin{align}
		% 	 	I(\phi,f)= &\sup_{|\phi| \leq 1}\left(\mathbb{E}[\hat I_N(\phi) \!-\! {I_N(\phi)}] \right)\nonumber
		% 	 	\\
		% 	 	&-\sup_{f \in \mathcal{F} }\left(\mathbb{E}[\hat I_N(f) \!-\! {I_N(f)}] \right).
		% 	 \end{align}
		%
		%  Note that for a special case when the test function lies  in $\mathcal{F}$, the approximation error $I(\phi,f)=0$. For other general functions, we assume a constant upper bound on $I(\phi,f)\leq \mathcal{Z}$
		Following Assumption \ref{as:approximation}, we could write \eqref{IPM0} as 
		%
		\begin{align}\label{IPM00}
			\sup_{|\phi| \leq 1} \left(\mathbb{E}[\hat I_N(\phi) \!-\! {I_N(\phi)}] \right)
			=&\sup_{f \in \mathcal{F} }\left(\mathbb{E}[\hat I_N(f) \!-\! {I_N(f)}] \right)+\mathcal{Z}.
		\end{align}
		%
		
		Note that the first term on the right hand side of \eqref{IPM00} describes the instance of an integral probability metric (IPM) [Muller 1997] given by
		%
		\begin{align}\label{IPM1}
			\sup_{f \in \mathcal{F} } &\left(\mathbb{E}[\hat I_N(f) \!-\! {I_N(f)}] \right)\nonumber
			\\
			&=\sup_{f \in \mathcal{F} } \left(\int f(\bbx)d\hat \mu_N -\int f(\bbx)d\tilde\mu_N\right)
	\end{align} }
	%
	%
	\blue{where $\hat\mu_N$  is the pre-image unnormalized density estimate obtained by solving \eqref{eq:proximal_hilbert_representer}. The IPM in \eqref{IPM1} is exactly equal Maximum Mean Discrepancy (MMD)\cite{fortet1953convergence,muller1997integral}. Hence, we could write }
	%
	\blue{\begin{align}\label{eq:mmd}
			%
			\sup_{f \in \mathcal{F} } \left(\mathbb{E}[\hat I_N(f) \!-\! {I_N(f)}] \right) =\|\beta_{ N}-\gamma_{N}\|_{\mathcal{H}}.
			%
	\end{align}}
	%
	\blue{where $\gamma_{N}$ is the kernel mean embedding corresponding to the uncompressed measure estimate $ \tilde\mu_N$. Next, let us consider the term $\|\beta_{ N}-\gamma_{N}\|_{\mathcal{H}}$ and add subtract the per step uncompressed estimate $\tilde\beta_{N}$ [cf. \eqref{eq:importance_sampling_stack2}] to obtain
	}
	%
	\blue{\begin{align}\label{triangle}
			\|\beta_{N}-\gamma_{N}\|_{\mathcal{H}} =& \|(\beta_{ N}-\tilde\beta_{ N})+(\tilde\beta_{ N}-\gamma_{N})\|_{\mathcal{H}}\nonumber
			\\
			\leq & \|\beta_{ N}-\tilde\beta_{N}\|_{\mathcal{H}}+\|\tilde\beta_{ N}-\gamma_{\nu_N}\|_{\mathcal{H}}\nonumber
			\\
			\leq &  \epsilon_N+\|\tilde\beta_{N}-\gamma_{N}\|_{\mathcal{H}}
	\end{align}}
	%
	\blue{where the last inequality holds from the fact that $\|\beta_{N}-\tilde\beta_{ N}\|_{\mathcal{H}}\leq \epsilon_N$ (cf. Algorithm \ref{alg:komp}). Now we substitute the values of $\tilde\beta_{N}$ and $\gamma_{N}$ using the update in \eqref{eq:kernel_mean_emb2}, we get }
	%
	\blue{\begin{align}\label{triangle2}
			\|\beta_{ N}-\gamma_{N}\|_{\mathcal{H}}
			\leq &  \epsilon_N+\|\beta_{ {N-1}}-\gamma_{{N-1}}\|_{\mathcal{H}}.
	\end{align}}
	%
	Using the above recursion, we could obtain
	%
	\blue{\begin{align}\label{triangle3}
			\|\beta_{ N}-\gamma_{N}\|_{\mathcal{H}}
			\leq &  \sum_{n=1}^{N}\epsilon_n.
		\end{align}
		as stated in Theorem \ref{thm:main_result}. Hence, using the upper bound of \eqref{triangle3} into \eqref{eq:mmd}, and then we an write the final upper bound in \eqref{new4} as 
		%
		\begin{align}\label{new5}
			%
			\big|\sup_{|\phi| \leq 1}  \big(\mathbb{E}[\hat I_N(\phi)- I(\phi)] \big) \big| \leq  \sum_{n=1}^{N}\epsilon_n+\frac{24}{N} \rho +\mathcal{Z}.
			%
		\end{align}}
\end{myproof}

\blue{Next, we present the main result of this paper. }
    
%
%Observe, however, that for consistency \eqref{eq:consistent}, we require that the number of generated particles from the importance distribution and the parameterization of the importance distribution to be equal $\{\bby_u\}$, i.e. $M_n=n$. Therefore, for streaming settings where the number of observations is to be infinite, i.e., $t\rightarrow \infty$, we require infinitely many samples $\{\bbx^{n} \}$ from the importance distribution, whose parameterization in terms of samples $\bbx^{n}$ becomes infinite. The question, then, is how do we obtain estimators for \eqref{eq:template_problem} which are \emph{nearly} consistent but of finite memory.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%T  H  E  O  R  E  M%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Theoretical guarantees for Compressed Internalized IS (CKIS) }
\blue{\begin{theorem}\label{thm:main_result}
%
%  Suppose $\pi$, the proposal distribution is absolutely continuous with respect to $q$, the population posterior, and both are probability measures defined over $\ccalX$. Then they are related by their Radon-Nikodyn derivative:
%$$
%\frac{d q}{d \pi}(x) : = \frac{g(x ) }{\int_{\ccalX} g(x) \pi(dx)}
%$$
%where $g$ is the unnormalized density (Radon-Nikodyn derivative) of $q$ with respect to $\pi$. Define the second moment of the Radon-Nikodyn derivative as 
%%
%$$\rho:= \frac{\pi(g^2)}{\mu(g^2)}$$
%%
Let $\rho$ as in Lemma \ref{lemma} under Assumptions \ref{as:first}-\ref{as:approximation}, then 
%

1) for diminishing compression budget $\epsilon_n=\alpha^n$ with $\alpha=(0,1)$, the estimator of Alg. \ref{alg:compressed_online_kernel_importance_sampling} satisfy
%
%
\begin{align}\label{diminish}
	%
	\big|\sup_{|\phi| \leq 1}  \big(\mathbb{E}[\hat I_N(\phi)- I(\phi)] \big) \big| \leq  \frac{\alpha}{1-\alpha}+\mathcal{O}\left(\frac{1}{N}\right) +\mathcal{Z}.
	%
\end{align}
%
To obtain $\delta$ accurate integral estimate, we need $N\geq\mathcal{O}\left(\frac{1}{\delta}\right)$ and $0<\alpha\leq 1/(1+(2/\delta))$.

2) for constant compression budget $\epsilon_n=\epsilon>0$ and memory $\mathcal{M}:=\mathcal{O}\left(\frac{1}{\epsilon^{1/(2p)}}\right)$
%
\begin{align}\label{final0}
	%
	\big|\sup_{|\phi| \leq 1}  \big(\mathbb{E}[\hat I_N(\phi)- I(\phi)] \big) \big| \leq \mathcal{O}\left(\frac{N}{\mathcal{M}^{1/2p}}+\frac{1}{N}\right)
	%
\end{align}
and
\begin{align}
	\mathcal{O}\left(\frac{1}{\delta}\right)\leq N\leq \mathcal{O}\left(\delta {\mathcal{M}^{1/(2p)}}\right),
\end{align}
which implies that $\mathcal{M}\geq\mathcal{O}\left(\frac{1}{\delta^{4p}}\right)$. 
\end{theorem}}
\begin{myproof}
%
Consider the statement of Lemma \ref{lemma} and to proceed next, we characterize the behavior of term $\sum_{n=1}^{N}\epsilon_n$ since it eventually determines the final bias in the integral estimation. 

1) \blue{Diminishing compression budget: Let us consider $\epsilon_n=(\alpha)^n$ with $\alpha=(0,1)$, which implies that
%
\begin{align}\label{diminishing}
\sum_{n=1}^{N}\epsilon_n= \frac{\alpha(1-\alpha^N)}{1-\alpha}\leq \frac{\alpha}{1-\alpha}.
\end{align}
%
Substituting \eqref{diminishing} into the right hand side of \eqref{new5}, we get
%
\begin{align}\label{new6}
	%
	\big|\sup_{|\phi| \leq 1}  \big(\mathbb{E}[\hat I_N(\phi)- I(\phi)] \big) \big| \leq  \frac{\alpha}{1-\alpha}+\frac{24}{N} \rho.
	%
\end{align}
%
To obtain $\delta$ accurate integral estimate, we need $N\geq\frac{48\rho}{\delta}$ and $0<\alpha\leq 1/(1+(2/\delta))$.}

%

2) \blue{Constant compression budget: Let us consider $\epsilon_n=\epsilon$, which implies that
	%
	\begin{align}\label{constant_epsilon}
		\sum_{n=1}^{N}\epsilon_n= N\epsilon.
	\end{align}
Using \eqref{constant_epsilon} into \eqref{new5}, we can write
%
\begin{align}\label{final}
	%
	\big|\sup_{|\phi| \leq 1}  \big(\mathbb{E}[\hat I_N(\phi)- I(\phi)] \big) \big| \leq  N\epsilon+\frac{24}{N} \rho.
	%
\end{align}
For a constant compression budget $\epsilon$, from Theorem \ref{thm:model_order}, we have 
%
\blue{\begin{align}
		M_{\infty}\leq \mathcal{O}\left(\frac{1}{\eps^{2p}}\right):=\mathcal{M}.
\end{align}}
}
\blue{If we are given with a maximum memory requirement $\mathcal{M}$, then we could obtain the value of compression budget we need to choose $\epsilon$ as  
%
\begin{align}
	\epsilon=\frac{G}{\mathcal{M}^{1/(2p)}}
\end{align}
where $G$ is the bound on the unnomalized weight $g(x(u))\leq G$ for all $u$. Using this lower bound value of $\epsilon$ into \eqref{final}, we get
%
\begin{align}\label{final1}
	%
	\big|\sup_{|\phi| \leq 1}  \big(\mathbb{E}[\hat I_N(\phi)- I(\phi)] \big) \big| \leq \frac{NG}{\mathcal{M}^{1/2p}}+\frac{24}{N} \rho.
	%
\end{align}}
%
\blue{Note that the first term in the above expression increases with $N$ and the second term decreases with $N$, hence we obtain a tradeoff between memory and accuracy for the importance sampling based estimator. For a given memory $\mathcal{M}$ (number of elements we could store in the dictionary) and the required accuracy $\delta$, we obtain the following bound on the number of iterations $N$ 
%
\begin{align}
	\frac{48\rho}{\delta}\leq N\leq \frac{\delta {M^{1/(2p)}}}{2G},
\end{align}
%
which implies that for the increased accuracy we need to run for more iterations but we need more memory  and vice versa.    }
\end{myproof}
%
%$\hfill \blacksquare$

Theorem \ref{thm:main_result}  establishes that the compressed kernelized importance sampling scheme proposed in Section \ref{sec:algorithm} is \emph{nearly} asymptotically consistent, and can be made arbitrarily close to exact consistency by sending the compression budget $\epsilon_n$ to null. However, when these parameters are fixed positive constants, they provide a tunable tradeoff between bias and memory. That is, when the compression budget is a positive constant, then the memory of the posterior distribution representation is finite, as we formalize next. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%T  H  E  O  R  E  M%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  
\begin{theorem}\label{thm:model_order}
%
 Under Assumptions \ref{as:first}-\ref{as:2} (in Appendix \ref{apx_technicalities}), for compact feature space $\ccalX$ and bounded importance weights $g(\bbx^{(n)})$, the model order for Algorithm \ref{alg:compressed_online_kernel_importance_sampling}, $ M_n<\infty$ for all $n$ given by
%
\blue{\begin{align}
		M_{\infty}\leq \mathcal{O}\left(\frac{1}{\eps^{2p}}\right).
\end{align}}
%
\end{theorem}
%
Theorem \ref{thm:model_order} (proof in Appendix \ref{third_proof}) contrasts the classical bottleneck in the number of particles required to represent an arbitrary posterior, which grows unbounded \cite{agapiou2017importance}. While this is a pessimistic estimate, experimentally we observe orders of magnitude reduction in complexity compared to exact importance sampling, which is the focus of the subsequent section.
%Classically, the bandwidth $h$ goes to null with $N$ \cite{silverman2018density,zhang1996nonparametric}, which is not the case here.

